Towards a data-driven and scalable approach for window operation detection in multi-family residential buildings

Natural cooling, utilizing non-mechanical cooling, presents a low-carbon and low-cost way to provide thermal comfort in residential buildings. However, designing naturally cooled buildings requires a clear understanding of how opening and closing windows affect occupants' comfort. Predicting when and why occupants open windows is a challenging task, often relying on specialized sensors and building-specific training data. This limits the scalability of natural cooling solutions. Here, we, propose a novel unsupervised method that utilizes easily deployable off-the-shelf temperature and humidity sensors to detect window operations. The effectiveness of our approach is evaluated using an empirical dataset and compared with a state-of-the-art support vector machine (SVM) model. The results demonstrate that our proposed method outperforms the SVM on key indicators, except when indoor and outdoor temperatures have small differences. Unlike the SVM's sensitivity to time series characteristics, our proposed method relies solely on indoor temperature and exhibits robust performance in pilot studies, making it a promising candidate for developing a highly scalable and generalizable window operation detection model This work demonstrates the potential of unsupervised data-driven methods for understanding window operations in residential buildings. By enabling more accurate modeling of naturally cooled buildings, our work aims to facilitate the widespread adoption of this low-cost and low-carbon technology.

==> sections/archives.tex <==
% ## Formerly in Methods 

% To develop an understanding of how the indoor and ambient quantities of
% interest changed across the different experiments, we examined the
% distributions of the data. The internal relative humidity was higher
% than the ambient relative humidity across experiments. The temperature
% distributions, which had distinctive fluctuations across experiments,
% are shown in Figure~\ref{fig-data-collected}. We observe that experiment
% B had the widest distribution of indoor temperatures. Experiment C had
% internal temperatures that were higher and closer to the mean of the
% ambient temperatures. This can be attributed to higher ambient
% temperatures that were recorded during this time period, which makes for
% a particularly interesting edge case.


% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/dist_expa.png}
%          \caption{}
%          % \label{}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/dist_expb.png}
%          \caption{}
%          % \label{fig:three sin x}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/dist_expc.png}
%          \caption{}
%          % \label{fig:five over x}
%      \end{subfigure}
%          \Description{Three graphs indicating temperature distributions for indoor and outdoor measurements}
%         \caption{Distributions of temperature across experiments}
%         \label{fig-data-collected}
% \end{figure}



% The following metrics were introduced by \cite{de_rautlin_de_la_roy_deep_2023} and represent window
% detection specific evaluation metrics. (FIX)
% \paragraph{Opening Accuracy} The opening accuracy is an average of scores
% given to each opening instance predicted by a window detection model. An
% opening instance is an interval on \(t\), such as
% \(t_{nk} = t_n, t_{n+1}, \dots , t_k\), where the final guess from the
% algorithm, \(I(t_{nk}) = 1\). An opening receives a score of 0 if it
% does not correspond to a a true opening:
% \(I(t_{nk}) = 1, W(t_{nk} = 0)\), and a score of 1 it perfectly
% corresponds to a true opening: \(I(t_{nk}) = 1, W(t_{nk} = 1)\). The
% score for a given predicted opening interval decreases by a penalty of
% 0.33 for each time step that does not align to a true opening.
% Therefore, a predicted opening interval \(I(t_{nk}) = 1\) that aligns a
% true opening interval will have a score of at most 0 if it extends for
% more than two times steps away from a true value. For the opening
% accuracy metric described by \cite{de_rautlin_de_la_roy_deep_2023}, the value for each opening
% interval are bounded at 0, and then are averaged to get the opening
% accuracy for an entire model. Here we also consider an unbounded opening
% accuracy where the score for a given interval is not bounded at 0 but is
% allowed to become negative. This unbounded metric provides clearer
% indication of how ``off'' models are, given that due to the unfavorable
% nature of some of the datasets collected, many models we examined
% actually had a bounded opening accuracy of 0.



% ### Formerly in Results

% Subigure~\ref{fig:oa} and Subigure~\ref{fig:uoa} display the performance on
% the opening and unbounded opening accuracy metrics. We observe that ST
% has a far higher performance for experiment A, a slightly better
% performance for experiment C, and a score of 0 for experiment B. The
% unbounded opening accuracy allows us to compare just how ``off'' models
% are. We see that ST performs ``less poorly'' than the SVM across all
% experiments. This suggests that ST predictions of when window states
% change are, on average, closer in time to reality than the predictions
% of the SVM models.
